The smarty4covid dataset and knowledge base: a framework enabling interpretable analysis of audio signals

Harnessing the power of Artificial Intelligence (AI) and m-health towards detecting new bio-markers indicative of the onset and progress of respiratory abnormalities/conditions has greatly attracted the scientific and research interest especially during COVID-19 pandemic. The smarty4covid dataset contains audio signals of cough (4,676), regular breathing (4,665), deep breathing (4,695) and voice (4,291) as recorded by means of mobile devices following a crowd-sourcing approach. Other self reported information is also included (e.g. COVID-19 virus tests), thus providing a comprehensive dataset for the development of COVID-19 risk detection models. The smarty4covid dataset is released in the form of a web-ontology language (OWL) knowledge base enabling data consolidation from other relevant datasets, complex queries and reasoning. It has been utilized towards the development of models able to: (i) extract clinically informative respiratory indicators from regular breathing records, and (ii) identify cough, breath and voice segments in crowd-sourced audio recordings. A new framework utilizing the smarty4covid OWL knowledge base towards generating counterfactual explanations in opaque AI-based COVID-19 risk detection models is proposed and validated.

==> Tables/main_questionnaire.tex <==
\begin{longtable}{|p{4.65cm}|p{0.25cm}|p{4cm}|p{0.8cm}|p{6.3cm}|}
\hline
Field name & \multicolumn{2}{p{5cm}|}{Description} & Type & Values \\*
\hline
\endfirsthead


\hline
Field name & \multicolumn{2}{p{5cm}|}{Description} & Type & Values \\*
\hline
\endhead

\hline 
\caption{Main questionnaire json file description (Part 2)} \\*
\endfoot

\hline
\caption{Main questionnaire json file description} \\*
\endlastfoot

% First part of the table
\multicolumn{5}{|c|}{\textbf{Part 1: COVID-19 related conditions}} \\*
\hline
participantid & \multicolumn{2}{p{5cm}|}{Participant's identification number.} & String & UUID \\*
 \hline
 submissionid &	\multicolumn{2}{p{5cm}|}{Questionnaire's Identification number.}	& String & UUID\\*
 \hline
 covid\_status	& \multicolumn{2}{p{5cm}|}{Tested for COVID-19.}	& String & \makecell[l]{"positive": Positive, \\ "negative": Negative, \\ "no": Not tested}\\*
 \hline
 pcr\_test &	\multicolumn{2}{p{5cm}|}{Tested with PCR.} & Bool &\\*
 \hline
 rapid\_test & \multicolumn{2}{p{5cm}|}{Tested with a Rapid Antigen test.} &	Bool &\\
 \hline
 self\_test	& \multicolumn{2}{p{5cm}|}{Tested with a Rapid Antigen Self test.} &	Bool & \\
 \hline
 test\_last\_3\_days & \multicolumn{2}{p{5cm}|}{Tested in the last 3 days.} & Bool & \\
 \hline
 last\_negative\_test\_date	& \multicolumn{2}{p{5cm}|}{Date of the last negative test.} & String &	"yyyy-mm-dd" \\
 \hline
 first\_positive\_test\_date &	\multicolumn{2}{p{5cm}|}{Date of the first positive test.}	& String &	"yyyy-mm-dd"\\
 \hline
 vaccination\_status &	\multicolumn{2}{p{5cm}|}{COVID-19 vaccination status.}	& String & \makecell[l]{"no": No, \\ "partially": One of two shots, \\ "fully": Fully, \\ "booster1": Fully and Booster dose,\\ "booster2": Fully and two Booster doses}\\
 \hline
 latest\_vaccination\_date	& \multicolumn{2}{p{5cm}|}{Date of the last vaccination dose.} & String & "yyyy-mm-dd"\\
 \hline
 hospitalization & \multicolumn{2}{p{5cm}|}{Whether the user was hospitalised for COVID-19.} & String & \makecell[l]{ "0": "No", \\ "1": "I am currently hospitalized", \\ "2": "Yes, discharged a week ago", \\ "3": "Yes, discharged more than a month ago"}\\
 \hline
 exposure\_to\_someone\_with\_covid	& \multicolumn{2}{p{5cm}|}{Whether the user was exposed to a confirmed COVID-19 case.} & String & "No" / "Maybe" / "Yes" \\
 \hline
 travelled\_abroad	& \multicolumn{2}{p{5cm}|}{Whether the user has travelled abroad the last 14 days.} & String & \makecell[l]{"0": No,\\ "1": Yes} \\
 \hline
 submission\_timestamp &	\multicolumn{2}{p{5cm}|}{Timestamp when the submission was received} & String & \\
\hline
% Add a page break
\pagebreak

% Second part of the table
\multicolumn{5}{|c|}{\textbf{Part 2: Symptoms and vital signs}} \\
\hline
sore\_throat & \multirow{16}{*}{\begin{sideways}Symptoms\end{sideways}} & Sore Throat & Bool & \\* 
 dry\_cough	&  &	Dry Cough	& Bool & \\*	
wet\_cough	& &	Productive Cough &	Bool &\\*
sputum & &	Sputum &	Bool &\\*
runny\_nose & &	 Nasal congestion &	Bool &\\*
breath\_discomfort	& &	Dyspnea &	Bool & \\*
has\_fever	& &	Fever &	Bool & \\*
tremble & &	Chills &	Bool	& \\*
fatigue	& &	Fatigue &	Bool	&\\*
headache & &	Headache &	Bool & \\*
dizziness & &	Dizziness/ confusion &	Bool & \\*
myalgias\_arthralgias	& &	Myalgias, arthralgias	& Bool & \\*
taste\_smell\_loss	& &	Loss of taste/smell	& Bool & \\*
diarrhea\_upset\_stomach	& &	Stomach upset/ Diarrhea	& Bool & \\*
sneezing & &		Sneezing	& Bool	& \\*
dry\_throat	& &	Dry Throat	& Bool	& \\*
\hline
oxymeter & \multirow{8}{*}{\begin{sideways}Vital Signs\end{sideways}} & Oximetry test & Bool & \\*
oxygenSaturation & &	Oxygen Saturation &	Int	& [60, 99]\\*
bpm	& &	Beats per minute (BPM)	& Int	& [30, 250]\\*
blood\_pressure\_meter	& &	Blood pressure test	& Bool	& \\*
systolic\_pressure	& &	Systolic Pressure &	Int &	[30, 260]\\*
diastolic\_pressure	& &	Diastolic Pressure & Int &	[30, 260] \\*
breath\_holding	& & Seconds of breath holding & Int &	[0, $\infty$)\\
\hline
leave\_bed & \multirow{6}{*}{\begin{sideways}Difficulty to\end{sideways}} & Leave Bed & Bool &\\*
leave\_home	& &	Leave Home &	Bool & \\*
prepare\_meal	& &	Prepare Meal & Bool & \\*
concentrate	& &	Concentrate	& Bool	& \\*
self\_care	& &	Self Care &	Bool & \\*
other\_difficulty & & Every day activites & Bool &\\*
\hline
% Add a page break
\pagebreak

% Third part of the table
\multicolumn{5}{|c|}{\textbf{Part 3: Smoking habits, anxiety level and working status}} \\
\hline
smoking & \multirow{9}{*}{\begin{sideways}Smoking habits\end{sideways}}	& Smoking status	& String &	\makecell[l]{"nev": Never smoked,\\"ex": Ex-smoker,\\ "yes": Smoker}\\*
years\_of\_quitting\_smoking & & Years of quitting smoking	& Int	& [0, $\infty$)\\*
years\_of\_smoking	& &	Years of smoking &	Int & [0, $\infty$) \\*
no\_cigarettes	& &	Number of cigarettes per day &	String & \makecell[l]{"1u": less than 1,\\ "10u": 1-10,\\ "20u": 11-20,\\"20o": more than 20}  \\*
vaping	& &	Vaping	& String & \makecell[l]{"0": No, \\"1": Yes}  \\*
\hline
anxiety	& \multicolumn{2}{p{5cm}|}{Level of anxiety about the pandemic} &	String & \makecell[l]{"0": None,\\"1": Low,\\"2": Moderate,\\"3": High,\\"4": Very High}\\*
\hline
working &	\multicolumn{2}{p{5cm}|}{Working Status} &	String	& \makecell[l]{"home": Working from home,\\*
"hospital": Working in hospital,\\*
"store": Working in an essential \\*goods store (pharmacy, supermarket),\\*
"social": Working in a service with increased \\* contact with the general public,\\*
"no": Not working}
\label{tab:main_questionnaire}
\end{longtable}
